Algebraic Proofs of Path Disconnectedness using Time-Dependent Barrier Functions

Two subsets of a given set are path-disconnected if they lie in different connected components of the larger set. Verification of path-disconnectedness is essential in proving the infeasibility of motion planning and trajectory optimization algorithms. We formulate path-disconnectedness as the infeasibility of a single-integrator control task to move between an initial set and a target set in a sufficiently long time horizon. This control-infeasibility task is certified through the generation of a time-dependent barrier function that separates the initial and final sets. The existence of a time-dependent barrier function is a necessary and sufficient condition for path-disconnectedness under compactness conditions. Numerically, the search for a polynomial barrier function is formulated using the moment-sum-of-squares hierarchy of semidefinite programs. The barrier function proves path-disconnectedness at a sufficiently large polynomial degree. The computational complexity of these semidefinite programs can be reduced by elimination of the control variables. Disconnectedness proofs are synthesized for example systems.

==> sections/box_model_meas.tex <==
\subsection{Path Feasibility}

\label{sec:box_feasible}
\urg{This section needs proofs, and might not need to exist at all. It might be best to skip directly to Section \ref{sec:box_infeasible}.}

New control-occupation measures $\sigma_i^\pm \in \Mp{[0, T] \times X}$ may be defined for each input channel $u_i, \ i = 1..n$. Assume that $x(t \mid x(0), u(\cdot))$ is a given system trajectory satisfying $u(t) = \{u_i( t)\}_{i=1}^n$ and  $\forall t \in [0, T]: u_i(t) \in [-1, 1]$ in each $i$. The control action can be split into positive and negative components $u^+_i(\cdot), u^-_i(\cdot): [0, T] \rightarrow [0, 1]$ under the relation $u(t) = u^+(t) - u^-(t)$.
Given an occupation measure $\mu \in \Mp{[0, T] \times X}$ supported on a distribution of system trajectories, the control-occupation measures may be defined for all subsets $A \times B \in [0, T] \times X$ as
\begin{subequations}
\label{eq:control_occupation}
\begin{align}
     \int_{A \times B} d \sigma^+_i(t,x) &= \int_{A\times B}  \max(0, u_i(t)) d \mu(t,x) \\
     \int_{A \times B} d \sigma^-_i(t,x) &= \int_{A\times B}  \max(0, -u_i(t)) d \mu(t,x).
\end{align}
\end{subequations}

The measures in \eqref{eq:control_occupation} satisfy a domination relation, in which there exists a nonnegative slack measure $\hat{\sigma}_i \in \Mp{[0, T] \times X}$ such that 
\begin{align}
    \forall i=1..N: \ \mu = \sigma^+_i + \sigma^-_i + \hat{\sigma}_i. \label{eq:domination_slack} 
\end{align}

For a general system with control-affine dynamics and $k$ input channels constrained to $[-1, 1]$
\begin{equation}
    \dot{x} = f(t,x,u) = f_0(t, x) + \sum_{i=1}^k f_i(t, x) u_i
\end{equation}

The Liouville equation with control-occupation measures $\sigma_i$ is \cite{majumdar2014convex}
\begin{equation}
\label{eq:liou_box_general}
\delta_T \otimes\mu_T  =  \delta_0 \otimes\mu_0 + (\partial_t + f_0 \cdot \nabla_x)^\dagger \mu + \sum_{i=1}^k (f_i \cdot \nabla_x)^\dagger (\sigma_i^+ - \sigma_i^-) \end{equation}


The divergence operator $\nabla_x \cdot v$ is equal to dynamics $\mathbf{1} \cdot \nabla_x v$. Each control-occupation measure $\sigma_i$ is absolutely continuous with respect to $\mu$. By the Jordan decomposition there exists nonnegative slack measures $\hat{\sigma}_i \in \Mp{[0, T] \times X}$ such that $\mu = \sigma_i + \hat{\sigma}_i$ for each $i$. 


\begin{prop}
There exists a path between $X_0$ and $X_1$ remaining entirely within $X$ in time $T$ if the following program has a solution:
\begin{subequations}
\label{eq:connect_box}
\begin{align}
     & \delta_T \otimes\mu_T  =  \delta_0 \otimes\mu_0 + (\partial_t )^\dagger \mu + \textstyle\sum_{i=1}^n 2\partial_{x_i})^\dagger (\sigma_i^+-\sigma_i^-) &  \label{eq:connect_box_liou}\\
     & \mu = \sigma_i^+ + \sigma_i^- + \hat{\sigma_i} \label{eq:connect_box_abscont} & \forall i = 1..n\\
      &\mu_0(X_0) = 1 &  \label{eq:connect_box_prob}\\
      &\mu_0 \in  \Mp{X_0}, \quad \mu_1 \in \Mp{X_1}&\\
      &\mu \in \Mp{[0, T] \times X} & \label{eq:connect_box_occ} \\
      &\sigma_i^+, \sigma_i^- \ \hat{\sigma_i}\in \Mp{[0, T] \times X} &  \forall i = 1..n \label{eq:connect_box_cont_occ}
\end{align}
\end{subequations}



\end{prop}

The infinite-dimensional programs \eqref{eq:connect_meas} and \eqref{eq:connect_box} will have the same result up to a scaling in $T$. \urg{prove? \cite{majumdar2014convex} is about Backwards Reachable Set, and is not exactly what we need.}

% Constraining $U$ to a box is a relatively mild restriction and does not affect infeasibility if $X_0$ and $X_1$ are truly disconnected. 


\urg{[probably delete this]
If the degree-$d$ relaxation of \eqref{eq:connect_box} is feasible, a degree-$d$ approximation to the control law $u_i(t,x)$ can be found. If $y_{\sigma_i, \leq d}$ are the moments of $\sigma_i$ in the relaxation and $\M_{\mu, \leq d}$ is the degree-$1-d$ moment matrix formed by moments of $\mu$, the coefficients of $u_i$ are approximately:

\begin{equation}
    y_{u_{i}} = \M_{\mu, \leq d}^{-1} \  y_{\sigma_i, \leq d}
\end{equation}

The moment matrix is full rank because $\mu$ is supported on trajectories (curves) rather than points (atoms). The recoverd $u$ from $y_{u_{i}}$ may not be feasible (control values may violate $u_i(t)\in [0, 1]$), but a sharper approximation may be found with postprocessing \cite{korda2014controller}.
}
% If \eqref{eq:connect_box} is feasible and $X_0, X_1$ are path-connected, then an approximate control $u(t)$ may be extracted



==> sections/contributions.tex <==
The contributions of this paper are:
\begin{itemize}
    \item A certificate of path-disconnectedness through the level sets of time-dependent barrier functions, extending previous work on time-independent barrier functions, and bypassing Slater conditions;
    \item Extensions such as unions of sets, time-state partitioning, and exponential time-dependent barrier functions;
    \item Experiments that demonstrate path-disconnectedness proofs on basic semi-algebraic sets.
\end{itemize}

==> sections/extensions.tex <==
\section{Extensions}

\urg{maybe dont discuss this}
\subsection{Unions}
Semialgebraic sets are the closure of basic semialgebraic sets under unions and projections. This section details how to implement Program \eqref{eq:altern_box} in the case where $(X, X_0, X_1)$ are all unions of basic semialgebraic sets. 
Assume that these sets are the union of $(N, N_0, N_1)$ components respectively:
\begin{align}
    X = \bigcup_{j=1}^N X^j & & X_0 = \bigcup_{j=1}^{N_0} X^j_0 & & X_1 = \bigcup_{j=1}^{N_1} X^j_1 
\end{align}

The disconnectedness program \eqref{eq:altern_box} with unions may be posed as,
\begin{subequations}
\label{eq:altern_box_union}
\begin{align}
    & \forall j = 1, \ldots, N_0: \nonumber\\
    &\qquad v(0, x) \geq 1 & \forall x \in X_0^j \label{eq:altern_box_union_init}\\
    & \forall j = 1, \ldots, N_1: \nonumber\\
    &\qquad v(T, x) \leq 0 & \forall x \in X_1^j \label{eq:altern_box_union_term}\\
    & \forall j = 1, \ldots, N: \nonumber\\
    &\qquad \partial_t v(t, x) - \textstyle\sum_{i=1}^n \partial_{x_i} v(t, x) - \textstyle\sum_{i=1}^n\zeta_i(t, x) \geq 0& \forall (t, x) \in [0, T] \times X^j \label{eq:altern_box_union_traj}\\
    &\qquad  2 \partial_{x_i} v(t, x) + \zeta_i(t, x) \geq 0 \label{eq:altern_box_union_cont}&  \forall i = 1 \ldots n, \ (t, x) \in [0, T] \times X^j \\
    &\qquad  \zeta_i(t, x) \geq 0 \label{eq:altern_box_union_slack}&  \forall i = 1 \ldots n, \ (t, x) \in [0, T] \times X^j \\
    & \zeta_i(t, x) \in C([0, T] \times X) & \forall i = 1 \ldots n\\ 
    &v(t, x) \in C^1([0, T] \times X) & 
\end{align}
\end{subequations}

Complicated shapes such as spirals and mazes may be formed by the union of basic components (such as ellipses or rectangles). Stone-Weierstrass approximations of these shapes by the level set of a single polynomial may require exceedingly high degree to describe. Unions offer a tractable alternative which may provide a certificate of feasbility or infeasibility at a low degree.




% Let $X^j$ for $j=1 \ldots N$ for $N$ finite be compact basic semialgebraic sets. The set $X = \cup_j X^j$ is a compact semialgebraic set formed by a countable union. 

% If each set $X^j$ has an occupation measure $\mu^j$, then the total occupation measures on $X$ is $\mu = \sum_j \mu^j$. The box model \eqref{eq:connect_box} likewise has control-occupation measures $\sigma_i = \sum_j \sigma_i^j$ and  $\hat{\sigma}_i = \sum_j \hat{\sigma}_i^j$. The alternate program imposes nonnegativity constraints \eqref{eq:altern_box_traj} and \eqref{eq:altern_box_cont} on each region $[0, T] \times X^j$.

% In the same manner the initial set and terminal sets may be unions such that $X_0 = \cup_j X^j_0, \ X_1 = \cup_j X^1_j$. The mass constraint would impose that $\sum_j \inp{1}{\mu_{0j}} = 1$

% [Will need to implement this feature]

% [nonnegative program]



